Temporally Robust Multi-Agent STL Motion Planning in Continuous Time

Signal Temporal Logic (STL) is a formal language over continuous-time signals (such as trajectories of a multi-agent system) that allows for the specification of complex spatial and temporal system requirements (such as staying sufficiently close to each other within certain time intervals). To promote robustness in multi-agent motion planning with such complex requirements, we consider motion planning with the goal of maximizing the temporal robustness of their joint STL specification, i.e. maximizing the permissible time shifts of each agent's trajectory while still satisfying the STL specification. Previous methods presented temporally robust motion planning and control in a discrete-time Mixed Integer Linear Programming (MILP) optimization scheme. In contrast, we parameterize the trajectory by continuous B\'ezier curves, where the curvature and the time-traversal of the trajectory are parameterized individually. We show an algorithm generating continuous-time temporally robust trajectories and prove soundness of our approach. Moreover, we empirically show that our parametrization realizes this with a considerable speed-up compared to state-of-the-art methods based on constant interval time discretization.

==> _Random.tex <==
\clearpage

The semantics of STL indicate whether a signal $x$ satisfies a specification $\phi$ or not via evaluation on its predicates. 
However, we wish to additionally specify how robustly a signal satisfies the specification. 
To that end, we define the asynchronous temporally robust quantitative semantics of STL. 
The asynchronous temporal robustness (ATR) indicates to what extent each signal within a predicate can be shifted in order to still satisfy a specification. Especially in the aforementioned multi-agent examples, where specifications of ``{\em Always, between 5 and 7.6 seconds, robot 1 and robot 2 should be $\epsilon$ close}'' might occur, this becomes critical as agents are subjected to individual delays or advancements.
As such, we build upon the definition of asynchronous temporal robustness (ATR) \cite{lindemann2022temporal} to allow for individual signal shifts (asynchronously) for each predicate, and apply this to our non-constant segmented trajectory of B\'ezier curves. 
\\\\
First, let $\mathcal{S}_p$ be the set of signals that appear in predicate $p$. Let $x^p$ be the relevant state vector for predicate $p$, defined as $x^p = \{x_k \in x | k \in \mathcal{S}_p \}$. Let $I_{k,i} = [h^0_{k,i},h^d_{k,i}]$ be the time-span of segment $i$ of signal $k$.
\begin{definition}[Predicate Asynchronous Temporal Robustness]
\label{def:p_ATR}
    We consider each signal in predicate $p$, and define ATR on a segment $i \in [0,N]$ of signal $k \in \mathcal{S}_p$ which defines the maximum extent each signal $l \in \mathcal{S}_p$, including $k$, may shift. 
    Additionally, we have to consider index $i$ being replaced by indices $j \in J$ that now overlap the original time-span of $i$ given the shift $\kappa_k$ on signal $k$.
    First, we define the time-shifted state $x^p_{\bar{\kappa}}$, with time shift $\bar{\kappa} := (\kappa_1,...,\kappa_m) \in \mathbb{R}^m, m = |\mathcal{S}_p|$ as 
    \begin{equation}
        x^p_{\bar{\kappa}}(t) := [x_1(t+\kappa_1),...,x_m(t+\kappa_m)].
    \end{equation}
    % indicating that the stacked shifted state is a state vector for which each signal $x_k$ is potentially shifted by a unique delay ($\kappa_k < 0$) or advancement ($\kappa_k > 0$).
    We can then define the ATR of predicate $p$ for segment $i$ of signal $k$ as
    \begin{multline}
    \label{eq:ATR^p}
        \theta^{p}_{k,i}(x) :=  \chi^{p}_{k,i}(x^p) \cdot \\
        \max\left\{\tau \ge 0 : \begin{array}{c} \forall \kappa_1,...,\kappa_m \in [-\tau,\tau], \\ \chi^{p}_{k,j}(x^p_{\bar{\kappa}}) = \chi^{p}_{k,i}(x^p), \forall j \in J\end{array} \right\},
    \end{multline}
    where $\chi_{k,j}^p$ is the characteristic function for a segment $j$ in the set $J$, which is defined as
    \begin{equation}
        J = \{j \in [0,N] \big\rvert \exists \kappa_k \in [-\tau,\tau] : I_{k,j} + \kappa_k \cap I_{k,i} \neq \varnothing \}
    \end{equation}
    indicating all segments of $k$ that now intersect or have intersected the original time span of segment $i$ under the time-shift $\kappa \in [-\tau,\tau]$, which includes $i$ itself. Consideration of $J$ ensures that $\forall t \in I_{k,i}, \theta^{p}_{k,i}(x)\big\rvert_{t} \leq \theta^{p}_{k,i}(x)$.
\end{definition}

Based on this definition of the ATR per segment of a signal $k$ on a predicate $p$, we can define the ATR of the temporal operators of the fragment in Eq. \eqref{eq:stl_fragment} \textcolor{red}{this would already need the lost temporal robustness due to segments, but then it gets very implementation-heavy}
\begin{equation}
\label{eq:ct_theta_temporal2}
\begin{aligned}
    \theta_{\Box_I p}(x) &:= \min_{k \in \mathcal{S}_p}(\min_{i \in [0,N], I_{k,i}\cap I \neq \varnothing}(\theta^{p}_{k,i}(x))), \\
    \theta_{\diamondsuit_I p}(x) &:= \min_{k \in \mathcal{S}_p}(\max_{i \in [0,N], I_{k,i} \cap I \neq \varnothing}(\theta^{p}_{k,i}(x))).
    % \theta_{\Box_I p}(x) &:= \min_{k \in \mathcal{S}_p}(\min_{i \in [0,N], z^{\text{temp}}_{k,i/I}=\top}(\theta^{p}_{k,i}(x,t)), \\
    % \theta_{\diamondsuit_I p}(x) &:= \min_{k \in \mathcal{S}_p}(\max_{i \in [0,N], z^{\text{temp}}_{k,i/I}=\top}(\theta^{p}_{k,i}(x,t)).
\end{aligned}
\end{equation}
We can then use the recursive rules on the binary operators
\begin{equation}
\label{eq:ct_theta_binary2}
\begin{aligned}
    % \theta_{\neg \phi}^{\pm}(x,t) &:= -\theta_p^{\pm}(x,t), \\
    \theta_{\phi_1 \land \phi_2}(x) &:= \min(\theta_{\phi_1}(x),\theta_{\phi_2}(x)), \\
    \theta_{\phi_1 \lor \phi_2}(x) &:= \max(\theta_{\phi_1}(x),\theta_{\phi_2}(x)),
    % \theta_{\phi_1 \mathcal{U}_{I} \phi_2}^{\pm}(x,t) &:= \max_{t' \in t+I}(\min(\theta_{\phi_2}^{\pm}(x,t'),\min_{t" \in [t,t')}(\theta_{\phi_1}^{\pm}(x,t")))),
\end{aligned}
\end{equation}
to obtain the ATR of a specification $\phi$ as $\theta^{\phi}(x)$.

We are now able to state our main theorem
\begin{theorem}[Soundness]
 On the limited fragment from Eq. \eqref{eq:stl_fragment}, the ATR of a specification $\phi$, $\theta^{\phi}(x)$, recursively obtained from $\theta^{p}_{k,i}(x)$ from Th. \ref{def:p_ATR} and the subsequent temporal and binary operators from Eq. \eqref{eq:ct_theta_temporal2} and Eq. \eqref{eq:ct_theta_binary2}, is upper-bounded by the specification ATR $\bar{\theta}^{\phi}(x,t)$ from \cite{lindemann2022temporal} $\forall t \in [t_0,t_f]$, meaning the definitions provided are sound.
\end{theorem}
\begin{proof}
    Note that $\theta^{p}_{k,i}$ from Def. \ref{def:p_ATR} defines the maximum time shift, $\tau$, where each signal in the predicate remains true when shifted by any $\kappa_i$ in the interval $[-\tau,\tau]$. The usage of the set $J$ indicates that while the index $i$ gets replaced temporally by other indices $j \in J$, that $\forall \kappa_1,...,\kappa_m \in [-\tau,\tau]$, these indices adhere to the characteristic function of segment $i$.
    
    First, assume $\chi^{p}_{k,i}(x) = 1$ so that $\theta^{p}_{k,i}(x) \geq 0$.
    \begin{itemize}
        \item For $|\kappa| > |\theta^{p}_{k,i}(x)|$, $\exists j \in J \enspace s.t. \enspace \chi^{p}_{k,j}(x^p_{\bar{\kappa}}) \neq \chi^{p}_{k,i}(x^p)$, which follows directly from Eq. \eqref{eq:ATR^p}, for which it is possible that $I_{k,j} + \kappa \cap I_{k,i} = \varnothing$, and hence introduces conservativeness.
        \item For $|\kappa| \leq |\theta^{p}_{k,i}(x)|$, it follows directly that $\chi^{p}_{k,i}(x^p_{\kappa})\big\rvert_{t} = 1, \forall t \in [t_0,t_f]$.
    \end{itemize}
    Next, assume $\chi^{p}_{k,i}(x) = -1$ so that $\theta^{p}_{k,i}(x) \leq 0$.
    \begin{itemize}
        \item For $\delta_k > \theta^{p}_{k,i}(x)$, it similarly follows that $\exists j \in J \enspace s.t. \enspace \chi^{p}_{k,j}(x^p_{\bar{\kappa}}) \neq \chi^{p}_{k,i}(x^p)$.
        \item For $\delta_k \leq \theta^{p}_{k,i}(x)$, it follows directly that $\chi^{p}_{k,i}(x^p_{\kappa})\big\rvert_{t} = -1, \forall t \in [t_0,t_f]$.
    \end{itemize}
    
    For $\theta_{\Box_I p}$, the ATR is the minimum of all segment ATRs of each signal in the predicate. Despite asynchronous shifts in signals, this ensures that $\chi^{p}_{k,j}(x_{\bar{\kappa}}^{p}) = \chi^{p}_{k,i}(x) \enspace \forall i : I_{k,i} \cap I \neq \varnothing, \forall k \in \mathcal{S}_p$ as we only consider the signal with the most restrictive shift. 
    For $\theta_{\diamondsuit_I p}$, notice that the definition of $\theta^{p}_{k,i}$ is conservative in that $\chi^{p}_{k,j}(x^p_{\bar{\kappa}},t) = \chi^{p}_{k,i}(x^p,t) \forall j \in J$ whereas we would only strictly require that  $\exists j \in J : I_{k,j} + \kappa \cap I_{k,i} \neq \varnothing$ for which $\chi^{p}_{k,j}(x^p_{\bar{\kappa}}) = \chi^{p}_{k,i}(x^p), \forall \kappa \in [-\tau,\tau]$.
    Additionally, $\theta^{p}_{k,i}$, $\theta_{\Box_I p}$, and $\theta_{\diamondsuit_I p}$ are conservative in that the temporal robustness $\forall t \in [h^0_i,h^d_i]$ is defined by $\theta^{p}_{k,i}$ which is actually an upper-bound, $\theta^{p}_{k,i}(x)\big\rvert_{t} \leq \theta^{p}_{k,i}(x), \forall t \in [h^0_i,h^d_i]$. 
    % For $\theta_{\diamondsuit_I p}$ the ATR is the minimum of the maximum ATR of each segment of each signal in the predicate. 
    % This represents the largest shift where the predicate can be true at some point within the given interval, even under asynchronous shifting. 
    The binary $\land$ and $\lor$ are trivial. Given the considered fragment of Eq. \eqref{eq:stl_fragment}, this concludes the proof.
\end{proof}

A remark is in place regarding the notion of synchronous or predicate temporal robustness in \cite{rodionova2021time,lindemann2022temporal}.

\begin{remark}
    When a predicate is dependent on a single signal, e.g. "{\em robot 1 in area A}", then the ATR for the predicate in Def. \ref{def:p_ATR} collapses to the predicate robustness. This is implemented using the counting procedure in \cite{rodionova2021time} with non-constant segment durations.
\end{remark}

% Note that if a predicate $p$ relies on one signal only, the definition of ATR collapses to the predicate-shift definition in \cite{rodionova2021time} which indirectly states to what extent the interval of the temporal operator, $I$, can be shifted to still adhere to the original specification.














% \section{Toy-Example}
% Define $\theta^{+}_{p}(x,t)$ as the positive/forward temporal robustness of predicate $p$ that indicates the maximum positive/forward time shift allowed in the signal such that the predicate does not change truth value
% \begin{equation}
%     \theta^{+}_{p}(x,t) = \chi_{p}(x,t)\max\{\tau \geq 0 | \forall t' \in [t,t+\tau], \chi_{p}(x,t') = \chi_{p}(x,t)\}
% \end{equation}
% where $\chi_{p}(x,t)$ is the indicator function of the predicate.
% Now, we can consider conjunctions and disjunctions, which we define as 
% \begin{equation}
%     \theta^{+}_{\phi_1 \land \phi_2}(x,t) = \min\{\theta^{+}_{\phi_1}(x,t),\theta^{+}_{\phi_2}(x,t)\}
% \end{equation}
% \begin{equation}
%     \theta^{+}_{\phi_1 \lor \phi_2}(x,t) = \max\{\theta^{+}_{\phi_1}(x,t),\theta^{+}_{\phi_2}(x,t)\}
% \end{equation}
% A problem arises when we wish to consider temporal operators such as the Always ($\Box_{I}$), and Eventually ($\diamondsuit_{I}$). Although these can be recursively defined from the Until operator, let us consider the Always and Eventually directly for clarity. Since we are considering continuous-time temporal robustness, we can define temporal robustness as
% \begin{equation}
%     \theta^{+}_{\Box_{I}\phi}(x,t) = \min_{t\in I}(\theta^{+}_{\phi}(x,t))
% \end{equation}
% \begin{equation}
%     \theta^{+}_{\diamondsuit_{I}\phi}(x,t) = \max_{t\in I}(\theta^{+}_{\phi}(x,t))
% \end{equation}
% where clearly, we take the $\min$ or $\max$ over the temporal robustness for all continuous time within the interval of the specification. Essentially, to define the temporal robustness (without considering optimizing for it), we wish to find $t$ where $\theta^{+}_{\phi}(x,t)$ is minimized or maximized. Continuous time causes this to not be a $\min$ or $\max$ operation over an array.





% \subsection{Intuition with an example}
% Consider the example with the Always operator below to gather some intuition on what the temporal robustness would do in continuous time for a discrete number of Bezier curves. 
% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/toy_example_temporal_robustness.pdf}
% \caption{Toy-example of Always staying within a certain range $x \in A$ for a certain time interval $[t_{lb},t_{ub}]$}\label{visina8}
% \end{figure}
% In this scenario, $t_i$ are continuous variables and to be optimized by the MILP. We can intuitively find that the temporal robustness is $\theta^{+}(x,t) = t_5 - \bar{I} \leq t_5 - t_4$ (although in reality, we would add the last part after $t_5$, we cannot evaluate this in closed-form linearly, and hence it is lost). Our objective is therefore
% \begin{equation}
%     J = \max_{h,r}(\min_{t\in I}(\theta^{+}_{\phi}(x,t)))
% \end{equation}
% and here is where the problem arises; we have nested $\min$ and $\max$ operators, where, due to the fact that we are considering continuous-time temporal robustness (a quantitative signal), the inner $\min$ operator is an optimization problem itself. When implementing this in a conventional way by taking the minimum value of $\theta^{+}(x,t), t\in I$ and maximizing this, we would invariably end up with the temporal robustness of the Eventually operator (we still maximize the forward temporal robustness and hence wish to place $t$ at the lower bound of $I$, $\underline{I}$).
% \\\\
% Because we are considering temporal robustness as a continuous-time signal, we can also not take conjunctions or disjunctions to deal with temporal operators (this works in the qualitative sense and in the discrete-time, continuous $\Delta T$ scenario).
% \\\\
% At the end of the day, I believe we are dealing with a nested minimax problem that would require something like bi-level optimization. 





% \subsection{Potential Workarounds}

% \subsubsection{\textbf{Not working}: limit $t$}
% Intuitively, one could propose to limit $t$ to be at the upper-bound of the interval $I$, $\bar{I}$, as positive temporal robustness of the Always operator is intuitively realized when $\theta^{+}_{\Box_{I}} = t_5 - \bar{I}$, however, this would lead to the adherence as if we have an Eventually operator where we adhere at the last second possible.

% \subsubsection{\textbf{Not working}: replace $\min$ with $\max$}
% We could of course also replace any $\min_{t\in I}(\theta^{+}_{\phi}(x,t))$ with a $\max_{t\in I}(-\theta^{+}_{\phi}(x,t))$ so that every operator in the cost is a $\max$ operator (as we wish to also maximize the temporal robustness, i.e. maximize the cost function). However, as the image below shows, we are still not dealing with an array over which we take the $\max$ or $\min$ (in the figure, only the third Bezier curve has a relevant temporal robustness. Maximizing $-\theta^{+}_{p}(x,t) = t - t_3$ would lead to placing both $t$ and $t_3$ as close to $\bar{I}$ as possible, not promoting the actual temporal robustness of the specification.
% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/toy_examples_single_overlap.pdf}
% \caption{Toy-example of Always staying within a certain range $x \in A$ for a certain time interval $[t_{lb},t_{ub}]$, now with only one overlapping Bezier curve}\label{visina8}
% \end{figure}

% \subsubsection{\textbf{Working}: fragment of STL}
% My original approach considers the fragment where we have Conjunctions or Disjunctions of Eventually and Always operators. We can define temporal robustness as something much easier.

% Let us first define how the adherence of a Bezier curve to a predicate. As we can only make statements about states between the start- and end-point of the Bezier curve, we define a binary variable $z^{\text{spat}}_i \in \{0,1\}$ that indicates whether all control points of a Bezier curve (including the start- and end-point) adhere to $\mu(x) \geq 0$.

% We then define a binary variable $z^{\text{temp}}_i \in \{0,1\}$ that indicates whether the Bezier curve encompasses the relevant time-interval of the temporal operator
% \begin{equation}
% \label{eq:parse_time}
%     z^{\text{temp}}_i = \top \iff h_i^{0} \leq \bar{I} \land h_i^{d} \geq \underline{I}
% \end{equation}
% where $\underline{I}$ and $\bar{I}$ are the lower- and upper bound of the specification. We then define the temporal robustness over the temporal operator. Due to the fact that the time range of a single temporal operator might be encompassed by multiple Bezier curves, we wish to find the minimum and maximum time of all Bezier curves that adhere both spatially (by being in the area of interest) and temporally (by encompassing the interval)
% \begin{align}
%     h_{\text{min}} &= \min\{h_i^0 | z^{\text{temp}}_i \land z^{\text{spat}}_i = \top, \forall i\in N\} \\
%     h_{\text{max}} &= \max\{h_i^0 | z^{\text{temp}}_i \land z^{\text{spat}}_i = \top, \forall i\in N\}.
% \end{align}
% We can then define the temporal robustness of the predicate $p$ at any time between $t \in [h_{\text{min}},h_{\text{max}}]$ as the difference between the bounds and $t$.
% Subsequently, we can define the temporal robustness for the temporal operator $\diamondsuit_{I}$ according to
% \begin{align}
%     \theta^{+}_{\diamondsuit_{I}\phi} &= h^{\phi}_{\text{max}} - \underline{I} \iff \max_{t\in I} (\theta^{+}_{\phi}(x,t)), t = \underline{I} \\
%     \theta^{-}_{\diamondsuit_{I}\phi} &= \bar{I} - h^{\phi}_{\text{min}} \iff \max_{t\in I} (\theta^{-}_{\phi}(x,t)), t = \bar{I}
% \end{align}
% and for $\Box_{I}$ according to
% \begin{align}
%     \theta^{+}_{\Box_{I}\phi} &= h^{\phi}_{\text{max}} - \bar{I} \iff \min_{t\in I} (\theta^{+}_{\phi}(x,t)), t = \bar{I} \\
%     \theta^{-}_{\Box_{I}\phi} &= \underline{I} - h^{\phi}_{\text{min}} \iff \min_{t\in I} (\theta^{-}_{\phi}(x,t)), t = \underline{I}
% \end{align}





% \subsection{Final thoughts}
% In short, it seems that as the formal, nested formulation of temporal robustness relies on taking the $\min$ or $\max$ over its continuous optimization variable, that we are dealing with a nested optimization. I believe we need a workaround for this, but I might be completely wrong. I have talked with some colleagues about this, and we could not figure it out either. I am wondering what you think.




% \clearpage
% \section{STL Encoding}

% We can write down the qualitative semantics of STL as
% \begin{align}
%     z_{p} &= \land_{i=0}^{N}(\land_{j=0}^{d}(\land_{k=1}^{n_{faces}}(b^{k}-H^{k}r_i^j - \epsilon ||H^{k}||_2 \geq 0))) \\
%     z_{\Box_{I}\phi} &= \land_{i=0}^{N}([h_i^0,h_i^d]\cap I \neq \varnothing \implies z_{\phi}) \\
%     z_{\diamondsuit_{I}\phi} &= \lor_{i=0}^{N}([h_i^0,h_i^d]\cap I \neq \varnothing \implies z_{\phi})   
% \end{align}

% now we need to write down the robust semantics of the STL fragment. 
% Assuming a continuous-time, general definition of the robust semantics, we can refer to \cite{rodionova2021time} from which we can state the predicate, Always, and Eventually semantics as follows
% \begin{align}
%     \theta^{+}_{p}(x,t) &= \chi_{p}(x,t)\max\{\tau \geq 0 | \forall t' \in [t,t+\tau], \chi_{p}(x,t') = \chi_{p}(x,t)\} \\
%     \theta^{+}_{\Box_{I}\phi}(x,t) &= \min_{t\in I}(\theta^{+}_{\phi}(x,t)) \\
%     \theta^{+}_{\diamondsuit_{I}\phi}(x,t) &= \max_{t\in I}(\theta^{+}_{\phi}(x,t))
% \end{align}

% However, this is for continuous-time temporal robustness where we can exactly evaluate the adherence to the specification (and the time range) at each point along the curve. Due to the Bezier parametrization, we can only make statements about temporal adherence at the end-points of the temporal Bezier curve. 

% For the Always operator, in \cite{rodionova2021time}, it is assumed we can express temporal robustness accurately via counting the discretization steps. Due to the potentially long duration of the Bezier curves, we cannot make this assumption. Instead, we define continuous-time temporal robustness on a discrete number of curves as
% \begin{align}
%     \theta^{+}_{\Box_{I}\phi}(x,t) &= \min_{h^0_i \in I}\theta^{+}_p - (\bar{I} - h^0_i)\\
%     \theta^{+}_{\diamondsuit_{I}\phi}(x,t) &= \max_{h^0_i \in I}\theta^{+}_p + (h^0_i - \underline{I})
% \end{align}
% where, for the Always operator, we subtract the duration from the last relevant control point within the time range to the upper bound of the specification and for the Eventually operator, we add the duration from the lower bound of the specification to the first relevant control point within the time range. This is shown in the figure below, which also highlights conservativeness that we cannot accommodate for (but which is upper-bounded by the maximum duration of the Bezier curve)
% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/toy_examples_temp_robust.drawio.pdf}
% \caption{Toy-example of Always (top) and Eventually (bottom) staying within a certain range $x \in A$ for a certain time interval $I$. Notice the underapproximation of the true temporal robustness due to the end-point properties of the Bezier curve (Lost).}\label{toy_eventually_always}
% \end{figure}

% \subsubsection{Implementation}
% For the implementation, we can still rely on the counting procedure from \cite{rodionova2021time} yet, due to the non-continuous time, we expand the 1's and 0's counter according to
% \begin{align}
%     c_i^1 = (c_{i+1}^1 + (h_i^d - h_i^0))z_t \\
%     c_i^0 = (c_{i+1}^0 - (h_i^d - h_i^0))z_t
% \end{align}
% where $(h_i^d - h_i^0)$ is the difference between the end and start point of the temporal Bezier curve, representing the duration of the Bezier curve. Keep in mind that we have now defined continuous-time temporal robustness on a discrete number of points.

% To actually implement this, we cannot simply constrain $\theta^{+}_{\phi} \geq 0$ and with the cost-term $\theta^{+}_{\phi}$ as, for the Always operator, the temporal robustness does not define behavior before the upper bound of the time-range $\bar{I}$. We would add the constraint
% \begin{align}
%     \min_{h_i^0 \in [0,\underline{I}]}\theta^{+}_{\Box_I \phi}(x,t) - \max_{h_i^0 \in [\bar{I}, \Delta T]} \theta^{+}_{\Box_I \phi}(x,t) \geq \bar{I} - \underline{I}
% \end{align}
% which constrains that the difference between $\theta^{+}$ at the control point \emph{on} or \emph{before} $\underline{I}$ and $\theta^{+}$ at the control point \emph{on} or \emph{after} $\bar{I}$ is greater or equal than the $\Delta I$. This seems like a trivial constraint but it is necessary as Bezier curves between these control points may lay outside the spatial requirement.
